Towards Rational Deployment of Multiple Heuristics in A*

The obvious way to use several admissible heuristics in A* is to take their maximum. In this paper we aim to reduce the time spent on computing heuristics. We discuss Lazy A*, a variant of A* where heuristics are evaluated lazily: only when they are essential to a decision to be made in the A* search process. We present a new rational meta-reasoning based scheme, rational lazy A*, which decides whether to compute the more expensive heuristics at all, based on a myopic value of information estimate. Both methods are examined theoretically. Empirical evaluation on several domains supports the theoretical results, and shows that lazy A* and rational lazy A* are state-of-the-art heuristic combination methods.

==> Makefile <==
%.pdf: %.tex
	pdflatex $<
	bibtex `echo $< | sed 's/\.tex//'`
	pdflatex $<

all: lazya.pdf

lazya.pdf: lazya.tex paper.bib

clean:
	rm -f *.aux *.log

distclean: clean
	rm -f lazya.pdf

